A Single-Layer Asymmetric RNN: Potential Low Hardware Complexity Linear Equation Solver

A single layer neural network for the solution of linear equations is presented. The proposed circuit is based on the standard Hopfield model albeit with the added flexibility that the interconnection weight matrix need not be symmetric. This results in an asymmetric Hopfield neural network capable of solving linear equations. PSPICE simulation results are given which verify the theoretical predictions. Experimental results for circuits set up to solve small problems further confirm the operation of the proposed circuit.

==> dataset_details.tex <==



\section{Dataset Details}

We utilized raw video sequence RAISE dataset, provided by [reference], to train our model for this binary classification problem, where 1 means “Split” whereas 0 means “Not Split”, taking QP value to be 22. The provided dataset contained approximately 800,000 CU blocks of size 64$\times$64 along with labels. We selected 200,000 64$\times$64 CU blocks and split them to get a dataset of 800,000 CU blocks of size 32$\times$32. Similarly, we generated the dataset for CU block size 16$\times$16 and 8$\times$8. Training + Validation dataset for each  type CU block size {64,32,16,8} contained total 800,000 samples with corresponding labels. We trained our model using the same dataset as mentioned in [ref] to propose an unbiased comparison of model’s training time, accuracy and complexity defined by number of trainable parameters. 
For testing purpose, we created our own dataset from raw image sequences\footnote{Raw sequences  obtained  from  http://ultravideo.cs.tut.fi/\#testsequences}, with the help of HM 16.9 encoder software, tuning encoder parameters such as CU depth and intra-coding depth to be one and adjusting maximum and minimum CU size {64,32,16,8} accordingly, to test the accuracy of our model for early termination of CU splitting.
